Formalizing Trust in Artificial Intelligence: Prerequisites, Causes and Goals of Human Trust in AI

Trust is a central component of the interaction between people and AI, in that 'incorrect' levels of trust may cause misuse, abuse or disuse of the technology. But what, precisely, is the nature of trust in AI? What are the prerequisites and goals of the cognitive mechanism of trust, and how can we promote them, or assess whether they are being satisfied in a given interaction? This work aims to answer these questions. We discuss a model of trust inspired by, but not identical to, sociology's interpersonal trust (i.e., trust between people). This model rests on two key properties of the vulnerability of the user and the ability to anticipate the impact of the AI model's decisions. We incorporate a formalization of 'contractual trust', such that trust between a user and an AI is trust that some implicit or explicit contract will hold, and a formalization of 'trustworthiness' (which detaches from the notion of trustworthiness in sociology), and with it concepts of 'warranted' and 'unwarranted' trust. We then present the possible causes of warranted trust as intrinsic reasoning and extrinsic behavior, and discuss how to design trustworthy AI, how to evaluate whether trust has manifested, and whether it is warranted. Finally, we elucidate the connection between trust and XAI using our formalization.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> section_nine_archive.tex <==
\section{Additional details behind our formalization, and future work}

\subsection{Elements of Trust in Social Science}


Section \ref{sec:trust-basic-definition} discusses a basic definition of trust in sociology which informs the rest of our work. %This definition of trust is considered overly simplistic in sociology.
In this section we discuss additional aspects of interpersonal trust and their relevance to \HumanAI trust.

\subsubsection{Trust vs Reliance} \label{subsec:reliance}

%A preliminary question we should ask is whether \HumanAI trust can even be considered trust from a perspective of sociology.
\citet{baier1986trust} introduces the term \textit{reliance} for trust in inanimate objects, such as trusting a stool to hold your weight. 
%\citet{baier1986trust} makes a distinction between trust and reliance, where reliance is considered to be a simpler variation of trust in inanimate objects, such as trusting a stool to hold your weight. %``I trust this stool to hold my weight.''
We may feel betrayed when our trust fails us, but this is not true for reliance because we did not attribute intent to the trustee \citep{tallant2020trust-commerce}. 
Despite the fact that AI models are tools, people anthropomorphize them and assign intent to them \citep{miller2017social, jacovi2020aligned-social}. This makes us believe that reliance is not suitable for AI models, and for this reason we aim to define \HumanAI \textit{trust} instead of reliance. This positions \HumanAI trust as a distinct sub-case of human-machine trust, or trust in automation, where the automation may not be attributed with intent (in which case, it is reliance). 
%As mentioned by \citet{miller2017social} and \citet{jacovi2020aligned-social}, humans do attribute human intent to AI models, so we elect to define human-AI trust as trust (rather than reliance), despite AI models being tools. However, more discussion in this area may be appropriate. 

\subsubsection{Warranted and Justified Trust in Social Science} \label{subsubsec:warranted-trust-social}

Our definition of warranted \HumanAI trust (\sect{sec:human_ai_definitions}) %, as mentioned,
is trust which is caused by trustworthiness (relative to some contract). This definition is only applicable to \HumanAI trust, and strictly speaking, is \textit{not} relevant in sociology. 

Sociology elects to define trustworthiness and \textit{justified} trust by the effect, rather than the cause: \textbf{in interpersonal trust, the trustee is trustworthy, and the trust in them was justified, if the trust was not betrayed}. Two natural questions emerge: (1) why does sociology define interpersonal trust in this way? (2) and why do we not adopt this definition for \HumanAI trust?

The \textit{capability} of the trustee to maintain the trust, and their \textit{intent} to do so, are both prerequisites to interpersonal trust, \textit{but not necessarily sufficient}. This is due to the complex nature of human interaction, with respect to elements of chance and outside factors (e.g., the difference between mistake and negligence, chains of trust, and so on). This makes the assignment of blame difficult or ill-defined. For example, if the trustee was fully capable of maintaining their trust, and intended to do so, but contracted a common cold which ultimately prevented them from achieving their goal---it is difficult to define them as trustworthy or otherwise. 

\HumanAI trust does not share these limitations, as (1) the AI (by definition as an automation) does not possess real intent; and (2) the AI's capabilities are well-defined. As a result, we diverge from sociology definitions on trustworthiness and warranted trust, and adopt a strict causal definition of warranted trust. 
%\ana{Someone may argue that we can consider the intent of the AI to be the intent of its developer using the same logic as in \S \ref{sec:trust-basic-definition} (trustee's incentives)?} \todo{I thought about this carefully and I think this definition is still good. The AI *by definition* does not possess intent, because it's a machine, so any trust following intent/incentives of the AI must be trust in the AI developer, and not the AI, and is simply not part of our modeling of Human-AI trust (even if it does, in the end, manifest in the interaction between the human and the AI, and we should recognize it in this work, which i added here below).}

% Still, the distinction between warranted and unwarranted trust %, of course,
% does apply in the AI case. For example, ``plausible but unfaithful'' explanations \citep{rudin2019stop,jacovi2020faithfulness}, where the explanation seems convincing to the user despite being unrepresentative of the model's true reasoning process, are one cause of unwarranted trust. \ana{Your ACL paper says that binary values for faithfulness are not practical (which I strongly agree with) and hence ``unfaithful'' could describe most explanations. Consider avoiding terminology ``plausible but unfaithful'', and just say: ``For example, explanations that seems convincing to the user despite being completely unrepresentitive of the model's true reasoning process, are one cause of unwarranted trust.''}



\subsubsection{Trust in the AI Developer}

\todo{like ana said, this subsection can be presented as area for future work, rather than "what we're not doing". i wrote it like this for now...}

Literature in sociology often considers aspects of larger social constructs (beyond a single transaction of two people), specifically relationships and communities and the propagation of trust in them. A common theme in such models is the incentives of both parties (e.g., trust in family vs trust in a business partner). 

This notion is, of course, relevant to \HumanAI trust. For example, since there is a close relationship between workplaces with discriminatory practices and discriminatory AI tools \citep{west2019discriminating}, it is likely that those who are discriminated against have more incentive to trust AI tools produced by teams that represent them. By recognizing the incentives of the developer, the user may gain trust in the AI.

The AI, as an automation, strictly speaking does not embody intent. Formally, the intent of the AI developer manifests in the capability of the AI to maintain specific contracts, rather than adopting some anthropomorphized notion of intent. Therefore, we make two claims on the nature of this trust:

\noindentparagraph{Trust in the AI based on trust in the AI developer is an instance of \textit{interpersonal} trust by proxy, and not \HumanAI trust.} Therefore,  studies of the influence of the trustee's incentives on \HumanAI trust, should build on the existing research in sociology that investigates the influence of relationships and communities on interpersonal trust \todo{cite some material}.

\noindentparagraph{Consequently, the question of whether this trust is \textit{warranted} or \textit{unwarranted} is ill-defined.} Our definition of warranted trust---as trust which is \textit{caused} by trustworthiness---is a definition that does not apply to interpersonal trust (as mentioned in \sect{subsubsec:warranted-trust-social}). 


To conclude, while trust in the AI developer \textit{could} possibly influence the interaction between the user and the AI, and should therefore be studied and modeled, it is strictly not part of our model of \HumanAI trust. \todo{please tell me if you agree with this, because if not, i'm willing to reconsider, but currently this is the only conclusion that makes sense to me.} \ana{This looks good to me!}


\subsection{Personal attributes of the trustor}

\todo{position as future work instead of "we don't do this"}

We additionally do not consider personal attributes of the trustor, such as personality or the prior existence of distrust (not to be confused with the absence of trust; see \citet{stanford-trust}), or the restoration of trust which has been betrayed. This is in the interest of generality in the scope of this work, and not necessarily representative of reality.  \ana{Be more explicit how we would need to narrow the scope if we considered distrust or restoration of trust, and whether there are any risks of not including these factors.} \todo{not sure i understand. we're not modeling the personal attributes because there's already enough work for us to do on the things that are general to all humans (and i don't think there's any risk in us doing it this way)}\ana{I am not sure that it is 100\% clear that distrust or restoration of trust from a previous interaction with AI does not affect how people trust that AI in the future (relevant for Section 7). I think it is fine to say that we ignore this case for simplicity and assume a ``clean slate'', but that this is not a realistic case in AI deployment. This makes me think we could have a discussion section in the end where we discuss all the assumptions we made and that these could be worked on in the future to create a more sophisticated definition and evaluation of trust, but that in this work we focus on providing a fundamental definition of \HumanAI trust that all of these additions can build on.}

\ana{Regarding personal attributes of the trustor. The paper ``Explainable AI for Cultural Minds'' {\small\url{https://kclpure.kcl.ac.uk/portal/files/134728815/DEXA_aug_crc.pdf}} studies the influence of user's socio-cultural background on their explanation needs. This may have influence on trust.}
% Finally, while we will take into account trust as a symptom of \textit{risk}, we consider precise discussion on vulnerability and risk to be beyond the scope of this work \todo{cite sociology on risk}. \ana{Be more explicit why it is outside of the scope of this paper.}

\subsection{Can trust become warranted?}

In this work, we discuss warranted trust as a `state' which trust can become, on a binary. This is equivalent to the notion of trust becoming `calibrated' as discussed by \citet{lee2004trust-calibrated}. Naturally, this is not strictly true in reality, as trust can increase or decrease freely---on a sliding scale. But is the sliding scale, in itself, sufficient to describe trust?
% Naturally, this is not strictly true in reality, as trust can increase, decrease, or morph and change freely. Strong trust can very swiftly change to strong distrust, and vice-versa. 

More specifically, \citet{hoffman2017taxonomy-trust-automation} argues that trust cannot be positioned on a binary, or even a sliding scale, as trust is multi-dimensional:
\begin{quote}
    In domains such as information technology security and weather forecasting, workers can depend on dozens of software suites, each offering multiple functionalities, some suites running on the same computer, some running on different computers or servers, some using the same operating system, and some using different operating systems. In my own relation to my word processing software, I am positive that it will perform well in the crafting of simple documents, but I am simultaneously confident it will crash when the document gets long, or when it has multiple high-resolution images. And every time that there is a software upgrade, the trusting of many of the functions becomes tentative and skeptical. [Therefore,] trust is not a single state.
\end{quote}
We contend that the argument of \citeauthor{hoffman2017taxonomy-trust-automation} is implicitly informed by a notion of contractual trust. In other words, \textbf{while general trust cannot be described by a single state (or sliding scale) of warranted or unwarranted, trust in a contract can,} since it is `calibrated' by the capability of the model to maintain the contract.


% \subsection{Trust in Automation}

% \todo{i think we can delete this section, because we address trust in automation in various points over the work. but it's still worth putting a footnote somewhere just to acknowledge this area as a father or precursor to human-ai trust.}

% \noindentparagraph{Trust in automation.} The subject of trust in automation can be seen as a precursor to trust in artificial intelligence, and has been discussed at length before \citep{parasuraman1997automation-use-misuse,hoffman2017taxonomy-trust-automation}. While AI models have many peculiarities that are seldom discussed in ``trust in automation'' literature, in particular the differentiation from reliance (the attribution of intent to the model) and the lack of transparency (often black-box models), some progress in those areas is certainly relevant to us, which we will consider as well. %\ana{Is this specific to social sciences?} \todo{what do you mean?} \ana{This paragraph didn't perfectly fit the section that was titled `Trust in social sciences'.}

